ToFu: Visual Tokens Reduction via Fusion for Multi-modal, Multi-patch, Multi-image Task

Large Multimodal Models (LMMs) are powerful tools that are capable of reasoning and understanding multimodal information beyond text and language. Despite their entrenched impact, the development of LMMs is hindered by the higher computational requirements compared to their unimodal counterparts. One of the main causes of this is the large amount of tokens needed to encode the visual input, which is especially evident for multi-image multimodal tasks. Recent approaches to reduce visual tokens depend on the visual encoder architecture, require fine-tuning the LLM to maintain the performance, and only consider single-image scenarios. To address these limitations, we propose ToFu, a visual encoder-agnostic, training-free Token Fusion strategy that combines redundant visual tokens of LMMs for high-resolution, multi-image, tasks. The core intuition behind our method is straightforward yet effective: preserve distinctive tokens while combining similar ones. We achieve this by sequentially examining visual tokens and deciding whether to merge them with others or keep them as separate entities. We validate our approach on the well-established LLaVA-Interleave Bench, which covers challenging multi-image tasks. In addition, we push to the extreme our method by testing it on a newly-created benchmark, ComPairs, focused on multi-image comparisons where a larger amount of images and visual tokens are inputted to the LMMs. Our extensive analysis, considering several LMM architectures, demonstrates the benefits of our approach both in terms of efficiency and performance gain.

==> qualitatives/18.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{lp{13cm}}
\toprule
\multicolumn{2}{c}{
\begin{tabular}{m{0.0em} r m{0.0em} r}
    \rotatebox[origin=l]{90}{$\mathtt{{<}img1{>}}$}
    & 
    \makecell{
         \includegraphics[width=2.5cm]{images/abo_imgs/b748d61e.jpg}
         \includegraphics[width=2.5cm]{images/abo_imgs/415ed1a3.jpg} 
         \includegraphics[width=2.5cm]{images/abo_imgs/ac368582.jpg}
         }
    &
    \rotatebox[origin=l]{90}{$\mathtt{{<}img2{>}}$}
    & 
    \makecell{
         \includegraphics[width=2.5cm]{images/abo_imgs/93f28744.jpg}
         \includegraphics[width=2.5cm]{images/abo_imgs/4c46feb8.jpg} 
         \includegraphics[width=2.5cm]{images/abo_imgs/86de7d0a.jpg}
         }
\end{tabular}}\\ 
\arrayrulecolor{gray}
\textbf{Prompt}: & Given the images of Product 1: $\mathtt{{<}img1{>}}$ and the images of Product 2: $\mathtt{{<}img2{>}}$, can you compare them in terms of \textcolor{RoyalBlue}{$\mathtt{{<}characteristic{>}}$}?\\ 
\arrayrulecolor{gray}\midrule
\textbf{Ground Truth}: & \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Additional Functions{>}}$}: & Product 1 has military time, Product 2 has a chronograph, Product 1 and Product 2 both have an alarm \\
\textcolor{RoyalBlue}{$\mathtt{{<}Design{>}}$}: & Product 1 has an octagon shape, Product 2 has a matte white resin case with a rose gold-tone top ring \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Target Audience{>}}$}: & Product 1 is designed for men, Product 2 is designed for women \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Dimensions{>}}$}: & Product 1's dimensions are not mentioned, Product 2's dimensions are not mentioned \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Weight{>}}$}: & Product 1 weighs 0.075 pounds, Product 2's weight is not mentioned \\
\textcolor{RoyalBlue}{$\mathtt{{<}Color{>}}$}: & Product 1 is Red, Product 2 is White/Rose Gold \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Water Resistance{>}}$}: & Both products are water resistant to 165 Feet (50m) \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Case Material{>}}$}: & Both products have resin cases \\
\textcolor{RoyalBlue}{$\mathtt{{<}Strap{>}}$}: & Product 1 has a red silicone strap, Product 2 has a matte white resin strap \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Backlight{>}}$}: & Both products have a backlight, but with a 3 second delay in Product 1 and no delay mentioned in Product 2 \\
\arrayrulecolor{black}\midrule
\textbf{InternVL2-4B Vanilla}: & \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Additional Functions{>}}$}: & The images of Product 1 and Product 2 are similar in that they both feature a digital display and a red strap. However, there are differences in their additional functions and design elements.

% **Differences:**

% 1. **Additional Functions:**
%    - Product 1 has an "ALARM CHRONO" function, which includes a water resistance feature of 165FT.
%    - Product 2 does not explicitly mention an alarm or chrono function in the image.

% 2. **Design Elements:**
%    - Product 1 has a black and red color scheme with a digital display showing the time and date.
%    - Product 2 has a rose gold and white color scheme with a digital display showing the time and date.

% In summary, while both products share a similar basic design and functionality, Product 1 includes an alarm and chrono feature with water resistance, whereas Product 2 does not explicitly show these features in the image. \\
\textcolor{RoyalBlue}{$\mathtt{{<}Design{>}}$}: & The images of Product 1 and Product 2 show the following differences in design:

1. **Color Scheme**:
   - Product 1 has a red case and bezel.
   - Product 2 has a rose gold case and bezel.

2. **Display**:
   - Product 1 has a digital display.
   - Product 2 has a digital display with a different color scheme.

3. **Branding**:
   - Product 1 has the branding "amazon essentials" on the back of the watch.
   - Product 2 also has the branding "amazon essentials" on the back of the watch.

4. **Buttons**:
   - Product 1 has a single button on the right side of the case.
   - Product 2 has a single button on the right side of the case.

5. **Functionality**:
   - Both products appear to have similar functionalities, but the specifics of the display and buttons might differ slightly.

Overall, the primary difference in design between Product 1 and Product 2 is the color scheme of the case and bezel. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Target Audience{>}}$}: & The two products in the images are both digital watches, but they have some differences in design and features.

% **Product 1:**
% - **Design:** This watch has a red strap and a red case. It has a digital display with a black background and white text.
% - **Features:**
%   - It is an alarm clock with a chronograph function.
%   - It has a water resistance of 165 feet.
%   - It has a mode button and a reset button.
%   - It has a large, clear display that shows the time, date, and other functions.

% **Product 2:**
% - **Design:** This watch has a white strap and a rose gold case. It also has a digital display with a black background and white text.
% - **Features:**
%   - It is an alarm clock with a chronograph function.
%   - It has a water resistance of 165 feet.
%   - It has a mode button and a reset button.
%   - It has a large, clear display that shows the time, date, and other functions.

% **Differences:**
% - **Color Scheme:** The first watch has a red strap and case, while the second watch has a white strap and rose gold case.
% - **Aesthetic Appeal:** The first watch has a more vibrant and sporty look due to the red color, while the second watch has a more elegant and sophisticated look with its rose gold case.
% - **Target Audience:** The first watch might appeal more to those who prefer a bold and sporty style, while the second watch might appeal more to those who prefer a classic and elegant style.

% In summary, both watches serve the same primary function as alarm clocks with chronograph features and have similar water resistance capabilities. However, they differ in their color schemes and aesthetic appeal, which may influence the target audience's preferences. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Dimensions{>}}$}: & The images of Product 1 and Product 2 are identical. Both show a digital alarm clock with a red strap and a black face. The dimensions of the watch are 165FT. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Weight{>}}$}: & The images of Product 1 and Product 2 are identical. Both show a digital wristwatch with a red strap and a rose gold case. The watch displays the time, day, and water resistance rating. \\
\textcolor{RoyalBlue}{$\mathtt{{<}Color{>}}$}: & The images of Product 1 and Product 2 both show a digital wristwatch with a red strap. However, there are differences in their color schemes and design details.

Product 1 has a red strap and a black watch face with a digital display. The text on the watch face includes "ALARM CHRONO," "SU MO TU WE TH FR SA," and "WATER RESIST 165FT."

Product 2 has a white strap and a rose gold or pinkish-gold watch face with a digital display. The text on the watch face includes "ALARM CHRONO," "TH," and "WATER RESIST 165FT."

In summary, the main differences are:
1. Strap color: Product 1 has a red strap, while Product 2 has a white strap.
2. Watch face color: Product 1 has a black watch face, while Product 2 has a rose gold or pinkish-gold watch face. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Water Resistance{>}}$}: & The images of Product 1 and Product 2 both show digital watches with a water resistance feature. However, there are differences in their design and color schemes.

% Product 1:
% - Color: Red
% - Water Resistance: 165FT

% Product 2:
% - Color: Pink
% - Water Resistance: 165FT

% Both products have the same water resistance rating of 165 feet. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Case Material{>}}$}: & The images of Product 1 and Product 2 both show a digital wristwatch with a rectangular face and a red strap. However, there are some differences in their case materials and design:

% 1. **Case Material**:
%    - Product 1 has a red case.
%    - Product 2 has a rose gold case.

% 2. **Design**:
%    - Product 1 has a more rugged and sporty design with a black bezel and a black face.
%    - Product 2 has a more elegant and modern design with a rose gold bezel and a white face.

% 3. **Display**:
%    - Both products have a digital display showing the time and day.
%    - Product 1 has a black background with white and gray text.
%    - Product 2 has a white background with black and gray text.

% 4. **Branding**:
%    - Both products have the "amazon essentials" branding on their cases.

% In summary, the main differences are the case material (red vs. rose gold) and the overall design aesthetic (sporty vs. elegant). \\
\textcolor{RoyalBlue}{$\mathtt{{<}Strap{>}}$}: & The images of Product 1 and Product 2 both show a digital wristwatch with a red strap. However, there are differences in the strap design and color. Product 1 has a red strap, while Product 2 has a white strap. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Backlight{>}}$}: & The images of Product 1 and Product 2 both show digital watches with a red strap. However, there are differences in their backlighting and design.

% Product 1 has a red backlight, while Product 2 has a pinkish backlight. Additionally, Product 1 has a black strap, whereas Product 2 has a white strap. \\
\arrayrulecolor{black}\midrule
\textbf{InternVL2-4B + \method}: & \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Additional Functions{>}}$}: & The two products have the same "Additional Functions" as both are water-resistant up to 165 feet. \\
\textcolor{RoyalBlue}{$\mathtt{{<}Design{>}}$}: & The design of the two products is different. Product 1 has a black and red color scheme with a digital display, while Product 2 has a white and pink color scheme with a digital display. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Target Audience{>}}$}: & The target audiences for the two products are different. Product 1 is designed for outdoor activities and water sports, indicated by the water resistance feature and the rugged design. Product 2 is designed for everyday wear and has a more fashionable appearance, indicated by the rose gold color and the brand name "amazon essentials." \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Dimensions{>}}$}: & The two products have different dimensions. Product 1 has a water resistance of 165 feet, while Product 2 has a water resistance of 38 feet. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Weight{>}}$}: & The weight of the two products is the same, as both are labeled with "165FT." \\
\textcolor{RoyalBlue}{$\mathtt{{<}Color{>}}$}: & The two products have different colors. Product 1 is red, while Product 2 is white. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Water Resistance{>}}$}: & Both products have the same water resistance rating of 165FT. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Case Material{>}}$}: & The case material of the two products appears to be different. Product 1 has a red case, while Product 2 has a white case. \\
\textcolor{RoyalBlue}{$\mathtt{{<}Strap{>}}$}: & The strap of Product 1 is red, while the strap of Product 2 is white. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Backlight{>}}$}: & The images of Product 1 and Product 2 both have a backlight feature, as indicated by the illuminated display on both watches. \\
\bottomrule
\end{tabular}
\end{table*}

==> qualitatives/31.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{lp{13cm}}
\toprule
\multicolumn{2}{c}{
\begin{tabular}{m{0.0em} r m{0.0em} r}
    \rotatebox[origin=l]{90}{$\mathtt{{<}img1{>}}$}
    & 
    \makecell{
         \includegraphics[width=2.5cm]{images/abo_imgs/2e1fd7bf.jpg}
         \includegraphics[width=2.5cm]{images/abo_imgs/2919d0ab.jpg} 
         \includegraphics[width=2.5cm]{images/abo_imgs/71bae565.jpg}
         }
    &
    \rotatebox[origin=l]{90}{$\mathtt{{<}img2{>}}$}
    & 
    \makecell{
         \includegraphics[width=2.5cm]{images/abo_imgs/f82a6ae8.jpg}
         \includegraphics[width=2.5cm]{images/abo_imgs/3c16f9e8.jpg} 
         \includegraphics[width=2.5cm]{images/abo_imgs/0e2ae917.jpg}
         }
\end{tabular}}\\ 
\arrayrulecolor{gray}
\textbf{Prompt}: & Given the images of Product 1: $\mathtt{{<}img1{>}}$ and the images of Product 2: $\mathtt{{<}img2{>}}$, can you compare them in terms of \textcolor{RoyalBlue}{$\mathtt{{<}characteristic{>}}$}?\\ 
\arrayrulecolor{gray}\midrule
\textbf{Ground Truth}: & \\
\textcolor{RoyalBlue}{$\mathtt{{<}Color Options{>}}$}: & Product 1 has Bronze Green, Product 2 has Black \\
\textcolor{RoyalBlue}{$\mathtt{{<}Style{>}}$}: & Product 1 is a running cap, Product 2 is a performance visor \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Gender{>}}$}: & Product 1 is for Men, Product 2 is for Women \\
\textcolor{RoyalBlue}{$\mathtt{{<}Product Type{>}}$}: & Product 1 is a running hat, Product 2 is a visor \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Material and Technology{>}}$}: & Both products use DRI-STAR technology and have a wicking sweatband, but the description does not provide information on the material used \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Size Option{>}}$}: & Both products have a one-size option \\
\arrayrulecolor{black}\midrule
\textbf{InternVL2-4B Vanilla}: & \\
\textcolor{RoyalBlue}{$\mathtt{{<}Color Options{>}}$}: & The images show two different styles of the same brand of hat, with the following differences in color options:

1. The first hat is in a dark green color.
2. The second hat is in a black color.

Both hats feature the same logo and design elements, but the primary color difference is between the two. \\
\textcolor{RoyalBlue}{$\mathtt{{<}Style{>}}$}: & The images of Product 1 and Product 2 both feature a star logo, but there are differences in their styles and colors.

**Product 1:**
- Color: Olive green
- Style: The star logo is white and appears to be embroidered on the front of the cap.
- Additional Features: The cap has a mesh back and a curved brim with a neon green trim.

**Product 2:**
- Color: Black
- Style: The star logo is also white and appears to be embroidered on the front of the cap.
- Additional Features: The cap has a similar curved brim with a neon green trim, but the overall color is black.

In summary, the main difference between the two products is the color of the cap: Product 1 is olive green, while Product 2 is black. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Gender{>}}$}: & The images of Product 1 and Product 2 both feature the "STARTER" logo, but they differ in color and design. Product 1 is olive green with a white star logo, while Product 2 is black with a white star logo. \\
\textcolor{RoyalBlue}{$\mathtt{{<}Product Type{>}}$}: & The images show two different types of caps:

1. The first cap is green with a white star logo and the word "STARTER" printed on it.
2. The second cap is black with a white star logo and the word "STARTER" printed on it.

Both caps have a similar design and branding, but the primary difference is the color of the fabric. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Material and Technology{>}}$}: & The images of Product 1 and Product 2 both feature a star logo, but there are differences in their design and color schemes.

% **Product 1:**
% - **Color Scheme:** Predominantly olive green with a neon green trim.
% - **Material:** Appears to be a combination of fabric and mesh, suggesting a blend of breathability and durability.
% - **Design:** The star logo is white and prominently displayed on the front. The cap has a structured design with a curved brim and a button on top.

% **Product 2:**
% - **Color Scheme:** Predominantly black with a neon green trim.
% - **Material:** Appears to be a solid fabric, likely providing a more uniform and possibly more durable surface.
% - **Design:** The star logo is white and is placed on the strap of the cap. The cap has a more streamlined and minimalist design with a flat brim and a single button on top.

% In summary, while both products share a star logo and neon green trim, Product 1 has a more complex design with a mix of fabric and mesh, and Product 2 has a simpler, more uniform fabric design. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Size Option{>}}$}: & The images show two different styles of the same brand of hat, with the following differences:

% 1. **Color**:
%    - The hat in the first image is olive green.
%    - The hat in the second image is black.

% 2. **Strap Design**:
%    - The hat in the first image has a bright lime green strap.
%    - The hat in the second image has a black strap.

% 3. **Strap Texture**:
%    - The strap in the first image appears to be smooth.
%    - The strap in the second image appears to be textured.

% 4. **Strap Material**:
%    - The strap in the first image looks to be made of a different material, possibly mesh or a similar fabric.
%    - The strap in the second image appears to be made of a different material, possibly a smoother, more solid fabric.

% 5. **Strap Design**:
%    - The strap in the first image has a simple, solid design.
%    - The strap in the second image has a more complex design with a star logo and additional text.

% These differences indicate that the two hats are variations of the same style, with different color options and strap designs available. \\
\arrayrulecolor{black}\midrule
\textbf{InternVL2-4B + \method}: & \\
\textcolor{RoyalBlue}{$\mathtt{{<}Color Options{>}}$}: & The images show two different color options for the same product, a baseball cap. Product 1 is in a green color, and Product 2 is in a black color. \\
\textcolor{RoyalBlue}{$\mathtt{{<}Style{>}}$}: & The style of the two products is different: Product 1 has a green color and a white star logo, while Product 2 has a black color and a white star logo with additional text. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Gender{>}}$}: & The images of Product 1 and Product 2 both feature a star logo on the front, but the color of the logo is different. Product 1 has a white star logo, while Product 2 has a black star logo. \\
\textcolor{RoyalBlue}{$\mathtt{{<}Product Type{>}}$}: & The two products are of the same type, both being baseball caps. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Material and Technology{>}}$}: & The two products appear to be the same, as they both feature the same star logo and brand name "STARTER." The primary difference is the color of the material: one is green and the other is black. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Size Option{>}}$}: & The images of Product 1 and Product 2 both feature a star logo on the front, but the color of the logo is different. Product 1 has a white star logo, while Product 2 has a black star logo. \\
\bottomrule
\end{tabular}
\end{table*}

==> qualitatives/53.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{lp{13cm}}
\toprule
\multicolumn{2}{c}{
\begin{tabular}{m{0.0em} r m{0.0em} r}
    \rotatebox[origin=l]{90}{$\mathtt{{<}img1{>}}$}
    & 
    \makecell{
         \includegraphics[width=2.5cm]{images/abo_imgs/a04951c7.jpg}
         \includegraphics[width=2.5cm]{images/abo_imgs/83eb6c69.jpg} 
         \includegraphics[width=2.5cm]{images/abo_imgs/8337e23c.jpg}
         }
    &
    \rotatebox[origin=l]{90}{$\mathtt{{<}img2{>}}$}
    & 
    \makecell{
         \includegraphics[width=2.5cm]{images/abo_imgs/bd03d7ae.jpg}
         \includegraphics[width=2.5cm]{images/abo_imgs/20533b83.jpg} 
         \includegraphics[width=2.5cm]{images/abo_imgs/8449b85e.jpg}
         }
\end{tabular}}\\ 
\arrayrulecolor{gray}
\textbf{Prompt}: & Given the images of Product 1: $\mathtt{{<}img1{>}}$ and the images of Product 2: $\mathtt{{<}img2{>}}$, can you compare them in terms of \textcolor{RoyalBlue}{$\mathtt{{<}characteristic{>}}$}?\\ 
\arrayrulecolor{gray}\midrule
\textbf{Ground Truth}: & \\
\textcolor{RoyalBlue}{$\mathtt{{<}Type of Product{>}}$}: & Product 1 is a combination of shampoo and body wash, while Product 2 is a single product of body wash, with a specific variant for men. \\
\textcolor{RoyalBlue}{$\mathtt{{<}Size of Shampoo/Bottle{>}}$}: & Product 1's shampoo is larger in size (28-fluid ounce) compared to Product 2's body wash (18-fluid ounce). \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Testing on Animals{>}}$}: & Both products are not tested on animals. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Scents{>}}$}: & Product 1 has a 'Cool Mist' scent for its body wash and no specific scent mentioned for its shampoo, while Product 2 has a 'Fresh Scent'. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Guarantee{>}}$}: & Product 2 has a satisfaction guarantee with a refund option within a year of purchase, while this information is not mentioned in Product 1's description. \\
\textcolor{RoyalBlue}{$\mathtt{{<}Quantity{>}}$}: & Product 1 has a larger quantity of items (four 28-fluid ounce bottles of shampoo and four 21-fluid ounce bottles of body wash) compared to Product 2 (one 18-fluid ounce bottle of body wash). \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Made in the USA{>}}$}: & Both products are made in the U.S.A. with U.S. and foreign components. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Comparison to Other Brands{>}}$}: & Both products invite the user to try their product if they like a specific brand (Tresemme for shampoo, Dial for body wash, and Old Spice for body wash), but Product 2's comparison is more specific to the scent variant. \\
\arrayrulecolor{black}\midrule
\textbf{InternVL2-4B Vanilla}: & \\
\textcolor{RoyalBlue}{$\mathtt{{<}Type of Product{>}}$}: & The images of Product 2 are of a red bottle of SOLMO Men's Body Wash. \\
\textcolor{RoyalBlue}{$\mathtt{{<}Size of Shampoo/Bottle{>}}$}: & The images of Product 2 are of a red bottle of SOLMO Men's Body Wash. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Testing on Animals{>}}$}: & The images of Product 2 are of a red bottle of SOLMO Men's Body Wash. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Scents{>}}$}: & The images of Product 2 are of a red bottle of SOLMO Men's Body Wash. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Guarantee{>}}$}: & The images of Product 2 are of a red bottle of SOLMO Men's Body Wash. \\
\textcolor{RoyalBlue}{$\mathtt{{<}Quantity{>}}$}: & The images of Product 2 show a red bottle of "Men's Body Wash" with a label that includes the following information:

- **Product Name**: Men's Body Wash
- **Description**: Fresh scent, Cleans without drying
- **Quantity**: 18 FL OZ (532 mL)
- **Warning**: For external use only. Avoid getting into eyes. If this happens, rinse thoroughly with water. Keep out of reach of children.
- **Ingredients**: Water, Sodium Laureth Sulfate, Sodium Chloride, Sodium Lauryl Sulfate, Fragrance, Cocamidopropyl Betaine, Citric Acid, Sodium Benzoate, Disodium EDTA, Methylchloroisothiazolinone, Methylisothiazolinone, Green 3, Red 33,
- **Distributed by**: Amazon.com Services, Inc. Seattle, WA 98109
- **Barcode**: 8 42379 15438 6
- **Lot Number**: L0018208BA

The label also includes a satisfaction guarantee statement and a contact number for customer service. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Made in the USA{>}}$}: & The images of Product 2 are of a red bottle of SOLMO Men's Body Wash. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Comparison to Other Brands{>}}$}: & The images of Product 2 are of a red bottle of SOLMO Men's Body Wash. \\
\arrayrulecolor{black}\midrule
\textbf{InternVL2-4B + \method}: & \\
\textcolor{RoyalBlue}{$\mathtt{{<}Type of Product{>}}$}: & The two products differ in the following ways:

1. **Type of Product**:
   - Product 1: Moisture Rich Shampoo
   - Product 2: Men's Body Wash

2. **Brand**:
   - Both products are from the brand SOLMO.

3. **Function**:
   - Product 1: Moisture Rich Shampoo is designed for hair care, specifically to provide moisture to the hair.
   - Product 2: Men's Body Wash is designed for body care, specifically for cleansing the body.

4. **Volume**:
   - Product 1: 28 FL OZ (828 mL)
   - Product 2: 18 FL OZ (532 mL)

5. **Additional Ingredients**:
   - Product 1: Contains Vitamin E.
   - Product 2: Contains Cocapric acid, Citric acid, Disodium EDTA, and other ingredients.

6. **Usage**:
   - Product 1: Used for hair washing.
   - Product 2: Used for body washing.

7. **Color**:
   - Product 1: Has a blue and white color scheme.
   - Product 2: Has a red and white color scheme.

8. **Additional Information**:
   - Product 1: Has a "Cool Mist" description.
   - Product 2: Has a "Fresh scent" description.

These differences highlight the distinct purposes and formulations of the two products. \\
\textcolor{RoyalBlue}{$\mathtt{{<}Size of Shampoo/Bottle{>}}$}: & The two products have different sizes. Product 1 is a 28 FL OZ (828 mL) bottle, while Product 2 is a 18 FL OZ (532 mL) bottle. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Testing on Animals{>}}$}: & The two products in the images are:

% 1. **Solimo Rich Body Wash**:
%    - **Testing on Animals**: No, the product is not tested on animals.

% 2. **Solimo Cool Mist Body Wash**:
%    - **Testing on Animals**: No, the product is not tested on animals. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Scents{>}}$}: & The two products have different scents. Product 1 is "Cool Mist Body Wash" with a "Cool Mist" scent, while Product 2 is "Men's Body Wash" with a "Fresh scent" and "Cleans without drying." \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Guarantee{>}}$}: & The two products have different guarantees. Product 1, the "SOLMO Moisture Rich Shampoo," has a guarantee that if you aren't satisfied within a year of purchase, you can request a refund for any reason. Product 2, the "SOLMO Men's Body Wash," does not have a visible guarantee on the label. \\
\textcolor{RoyalBlue}{$\mathtt{{<}Quantity{>}}$}: & The two products have different quantities. Product 1 is a 28 FL OZ (828 mL) bottle, while Product 2 is a 18 FL OZ (532 mL) bottle. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Made in the USA{>}}$}: & The two products in the images are both from the brand Solimo. However, they are different products:

% 1. The first product is Solimo Shampoo Rich Body Wash.
% 2. The second product is Solimo Men's Body Wash.

% Regarding the "Made in the USA" label, the Solimo Shampoo Rich Body Wash does not explicitly state "Made in the USA" on its packaging, while the Solimo Men's Body Wash does not have this information visible in the provided image. \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Comparison to Other Brands{>}}$}: & The two products have different scents:

% - Product 1: Rich Body Wash
% - Product 2: Men's Body Wash (Fresh scent) \\
\bottomrule
\end{tabular}
\end{table*}

==> qualitatives/82.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{lp{13cm}}
\toprule
\multicolumn{2}{c}{
\begin{tabular}{m{0.0em} r m{0.0em} r}
    \rotatebox[origin=l]{90}{$\mathtt{{<}img1{>}}$}
    & 
    \makecell{
         \includegraphics[width=2.5cm]{images/abo_imgs/89f7a20f.jpg}
         \includegraphics[width=2.5cm]{images/abo_imgs/fe45385c.jpg} 
         \includegraphics[width=2.5cm]{images/abo_imgs/35f5ea20.jpg}
         }
    &
    \rotatebox[origin=l]{90}{$\mathtt{{<}img2{>}}$}
    & 
    \makecell{
         \includegraphics[width=2.5cm]{images/abo_imgs/39270530.jpg}
         \includegraphics[width=2.5cm]{images/abo_imgs/25ca6802.jpg} 
         \includegraphics[width=2.5cm]{images/abo_imgs/f9d8dbb2.jpg}
         }
\end{tabular}}\\ 
\arrayrulecolor{gray}
\textbf{Prompt}: & Given the images of Product 1: $\mathtt{{<}img1{>}}$ and the images of Product 2: $\mathtt{{<}img2{>}}$, can you compare them in terms of \textcolor{RoyalBlue}{$\mathtt{{<}characteristic{>}}$}?\\ 
\arrayrulecolor{gray}\midrule
\textbf{Ground Truth}: & \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Item Name{>}}$}: & The product names are different - find. Fidel Derbys, Brown Classic Tan, 9 US for Product 1 and Amazon Brand - find. Women's Shoes with Plaited Leather and Gum Rubber Sole Moccasin for Product 2 \\
\textcolor{RoyalBlue}{$\mathtt{{<}Style{>}}$}: & Product 1 is a specific style (Fidel Derbys) whereas Product 2 is a more general style description (Find Women's Shoes With Plaited Leather and Gum Rubber Sole) \\
\textcolor{RoyalBlue}{$\mathtt{{<}Color{>}}$}: & Product 1 has a specific color mentioned (Brown Classic Tan) whereas Product 2 does not mention a specific color \\
\arrayrulecolor{black}\midrule
\textbf{InternVL2-4B Vanilla}: & \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Item Name{>}}$}: & The images of Product 2 are:

% 1. The first image shows a pair of brown leather dress shoes with a smooth finish and a classic design.
% 2. The second image shows a pair of brown leather sandals with a textured, crocodile skin pattern and a more casual design. \\
\textcolor{RoyalBlue}{$\mathtt{{<}Style{>}}$}: & The two products in the image are both brown leather sandals, but they differ in style. The first pair is a classic Oxford style with a closed lacing system and a low heel, while the second pair is a strappy sandal with a higher heel and a more open design. \\
\textcolor{RoyalBlue}{$\mathtt{{<}Color{>}}$}: & The two products in the image are both brown leather sandals. The first pair of sandals on the left is a classic Oxford style with a closed lacing system, while the second pair on the right is a strappy sandal with a more open design. \\
\arrayrulecolor{black}\midrule
\textbf{InternVL2-4B + \method}: & \\
% \textcolor{RoyalBlue}{$\mathtt{{<}Item Name{>}}$}: & The images show two different styles of shoes. Product 1 appears to be a classic lace-up shoe with a smooth leather finish, while Product 2 is a slip-on shoe with a textured leather design. \\
\textcolor{RoyalBlue}{$\mathtt{{<}Style{>}}$}: & The two products have different styles: Product 1 has a classic lace-up design, while Product 2 has a more casual, open-toe design with a woven texture. \\
\textcolor{RoyalBlue}{$\mathtt{{<}Color{>}}$}: & The two products have the same color. \\
\bottomrule
\end{tabular}
\end{table*}
